Evaluating the Diversity and Quality of LLM Generated Content

Recent work suggests that preference-tuning techniques -- such as Reinforcement Learning from Human Feedback (RLHF) methods like PPO and GRPO, as well as alternatives like DPO -- reduce diversity, creating a dilemma given that these models are widely deployed in applications requiring varied outputs. We argue that diversity without consideration of quality has limited practical value. To address this issue, we introduce a framework for measuring effective semantic diversity -- diversity among outputs that meet quality thresholds -- which better reflects the practical utility of large language models (LLMs). Using open-ended tasks that require no human intervention, we find counterintuitive results: when using diversity metrics that do not explicitly consider quality, preference-tuned models -- particularly those trained via RL -- often produce outputs with lower diversity; however, these same preference-tuned models generate greater effective semantic diversity than supervised fine-tuned (SFT) or base models. Our analysis further shows another trend: while larger models may exhibit greater effective semantic diversity than smaller models, the smaller models are consistently more parameter-efficient at producing unique content within a fixed sampling budget. These findings have practical implications for applications that require diverse yet high-quality outputs, from creative assistance to synthetic data generation.

==> latex/figures/all_cast_bar.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{latex/images/all_stripped_subtrees.png}
    \caption{All Distinct CAST}
    \label{fig:stripped_subtrees}
    
\end{figure*}

==> latex/figures/all_diversity_bar.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{latex/images/all_semantic_diversity.png}
    \vspace{0.5cm}
    \includegraphics[width=\textwidth]{latex/images/all_stripped_subtrees.png}
    \vspace{0.5cm}
    \includegraphics[width=\textwidth]{latex/images/all_distinct_n.png}
    \caption{Three stacked images: All Distinct N, All Distinct CAST, and All Distinct N-grams.}
    \label{fig:stacked_images}
\end{figure*}

==> latex/figures/all_ngrams_bar.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{latex/images/all_distinct_n.png}
    \caption{All Distinct N-grams}
    \label{fig:distinct_n}
\end{figure*}

==> latex/figures/all_semantic_bar.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{latex/images/all_semantic_diversity.png}
    \caption{All Semantic Diversity}
    \label{fig:semantic_diversity}
\end{figure*}

==> latex/figures/codebertscore_false_positives.tex <==
\begin{figure}[h]
\centering
% \begin{tcolorbox}[
%     width=0.98\textwidth,
%     colback=white,
%     colframe=black,
%     boxrule=1pt,
%     arc=0pt,
%     outer arc=0pt,
%     left=5pt,
%     right=5pt,
%     top=5pt,
%     bottom=5pt
% ]
    \begin{minipage}[t]{0.48\textwidth}
        % \textbf{Example 1: CodeBertScore: 0.9904}
        % \textsc{CodeBertScore}: 99.04
        \begin{minted}[fontsize=\footnotesize,frame=single,autogobble,breaklines]{python}
# CodeBertScore: 99.04
def f(A: int, B: int):
    print(A + B)

def f(A: int, B: int):
    print(A ^ B)
        \end{minted}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace{-0.5em}
        % \textcolor{black}{\rule{1pt}{5em}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        % \textbf{Example 2: CodeBertScore: 0.9878}
        % \textsc{CodeBertScore:} 98.78
        \begin{minted}[fontsize=\footnotesize,frame=single,autogobble,breaklines]{python}
# CodeBertScore: 98.78
def f(N: int, A: List[int]):
    print(min(A))

def f(N: int, A: List[int]):
    print(max(A))
        \end{minted}
    \end{minipage}
% \end{tcolorbox}
\caption{Examples where \textsc{CodeBertScore} fails to reflect execution semantics. Note we compare the program above to the program below. Both sets of programs are semantically different, but \textsc{CodeBertScore} is very high. The similarity scores are in the top $1^{\text{th}}$ percentile for all programs and, despite being semantically distinct, is also in the top $1^{\text{th}}$ percentile of the wrong class (of all semantically equal programs). }  

% \shuo{The current analysis is already convincing to me. I do not think it's necessary to compare the scores to those of all programs, as being smaller than scores between semantically different programs is less interesting.} 

% \alex{Make it clear it is top-bottom!!!! depends on what similarity means: ie for retrieval it is not insane }}

\label{fig:codebertscores-comparison}
\end{figure}

==> latex/figures/combined_corr.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{latex/images/combined_correlations_11-27_subsampled_0_30_ice_scores_and_codebert_f1_small.pdf}
    \caption{\textbf{Correlation between diversity metrics}: We analyzed the correlation of our diversity metrics across many experiments. We report the Spearman Rank Correlation and Kendall's Tau Rank Correlation Coefficients. }
    \label{fig:combined-corr}
\end{figure*}

==> latex/figures/dataset_creation_fig.tex <==
\begin{figure}[t]
    \centering
    {\color{blue}\framebox[\textwidth]{
        \includegraphics[width=0.99\textwidth]{latex/images/dataset_creation.pdf}
    }}
    \caption{\reb{A flow-chart of the creation process showing the steps from initial problem selection through final validation. The process involved manual of 1-shot examples, \texttt{gpt-3.5-turbo-0125}, manual review and selection of diverse problems, refinement of problem descriptions and test cases, and final validation.}}
    \label{fig:dataset_creation}
\end{figure}

==> latex/figures/llama3_temp_sweep.tex <==
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{latex/images/llama3_70b_instruct_temp_vs_diversity_metrics.pdf}
%     \caption{
%     % \textbf{It's all semantics!} 
%     We show the difference in diversity metrics when modulating the Temperature parameter for \textsc{Llama3-Instruct 70b}. Metrics that measure lexical or syntactic diversity increase with temperature, even as high-temperature outputs degenerate and become incoherent. }
%     \label{fig:temp-sweep}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \includegraphics[width=\textwidth]{latex/images/llama3_70b_instruct_temp_vs_diversity_metrics.pdf}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.48\textwidth}
%         % \centering
%         % \textbf{Lexical Diversity: 96.10\% \quad Syntactic Diversity: 88.89\%}
%         % \vspace{0.5em}
%         \begin{minted}[fontsize=\footnotesize,frame=single,autogobble,breaklines]{python}
% ## Lexical Diversity: 96.10%
% ## Syntactic Diversity 88.89%
% ## Semantically Equivalent: True

% def f(A: int, B: int):
%     C = A * B
%     print(C)

% def f(*args):
%     result = 1
%     for term in args:
%         result *= term
%     print(result)
%         \end{minted}
%     \end{minipage}
%     \caption{Left: Diversity metrics when modulating the Temperature parameter for \textsc{Llama3-Instruct 70b}. Metrics measuring lexical or syntactic diversity increase with temperature, even as high-temperature outputs become incoherent. Right: Two Python programs with different implementations, demonstrating high lexical and syntactic diversity despite being semantically equivalent in our dataset. Both generations from \textsc{MetaLLama3.1-70b-Instruct}}
%     \label{fig:diversity-and-programs}
% \end{figure}

\begin{figure}[!t]
\centering
\begin{minipage}{0.51\textwidth}
\vspace{4.5pt} 
\includegraphics[width=\textwidth]{latex/images/llama3_70b_instruct_temp_vs_diversity_metrics.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.47\textwidth}
\begin{minted}[fontsize=\scriptsize,frame=single,autogobble,breaklines]{python}
## Semantically Equivalent: True
## Lexical Diversity: 83.95%
## Syntactic Diversity (Height=4): 100.00%

def f(N: int, T: List[int]):
    print(sum(T))

def f(N: int, T):
    total = 0
    for num in T:
        total += num
    print(total)
\end{minted}
\end{minipage}
\caption{Left: Diversity metrics when modulating the Temperature parameter for \textsc{Llama3-Instruct 70b}. Metrics measuring lexical or syntactic diversity increase with temperature, even as high-temperature outputs become incoherent. Right: Two Python programs generated by \textsc{CodeLlama 7b} with different implementations, demonstrating high syntactic diversity and significant lexical diversity despite being semantically equivalent in our dataset. }.
\label{fig:diversity-and-programs}
\end{figure}



==> latex/sections/background_and_related.tex <==
%\section{Background and Related Work}

%\textbf{Automatic diversity evaluation.}
%
% Automatic evaluation of diversity is a relatively nascent area of NLP research: little work has systemically evaluated automatic metrics in capturing diversity, and none to our knowledge have evaluated their efficacy in evaluating the diversity of LLMs. Measuring LLM outputs may differ from human outputs given that models may be biased to machine-generated text \cite{NA} and outputs may fall outside the traditional distribution of training data. 

\textbf{Related work.}
Traditional methods for automatically measuring diversity fall into lexical or neural approaches. Lexical metrics generally involve calculating summary statistics using $n$-grams, such as \textbf{Distinct-N} \citep{distinct-n-2016, distinct_n_2019},
%the proportion of distinct $n$-grams in a corpus normalized by the total number of $n$-grams 
or \textbf{Self-BLEU} (a modified BLEU metric) \citep{self-bleu-texygen}. 
%that uses other sentences in a document as ``references" for a given sentence \citep{self-bleu-texygen}.
More recently, deep learning has been used to model similarity of natural language sentences \citep{bertscore-2019, sentence-bert-2019, openai-embeddings-2022} and code \citep{codebert-2020, codebertscore2023}; these techniques have been adapted to measuring diversity \citep{lai2020diversity, evaluating-the-evaluation-2021, nli-diversity-2021}. \citet{evaluating-the-evaluation-2021} compare lexical and neural metrics, finding that neural metrics outperform lexical ones, but still underperform humans. \citet{shaib2024standardizing} show that lexical diversity often captures the same information as traditional compression algorithms, and recommend reporting a combination of lexical and neural diversity scores. %However, \citet{shaib2024standardizing} recently observed that both lexical and neural metrics tend to be correlated with each other and with compression ratios obtained from traditional compression algorithms. \osbert{``More correlated'' compared to human evaluation?}


%Whatever prior work we have has indicated that lexical metrics and neural metrics substantially underperform humans in measuring diversity. \citet{evaluating-the-evaluation-2021}. Additional evidence has also pointed to phenomena that neural-network evaluation may bias in favor of machine-generated content \citep{storytelling-llms-xie-2023}. 

% However, despite these advances, relatively little work has systematically evaluated the reliability of these metrics in measuring the outputs of language models, \textit{especially when outputs are degenerate and outside of the usual distribution} of the training data. 


%Neural methods for evaluation open up opportunities for reward-hacking \cite{concrete-problems-safety-2016} and measurement bias, especially if using an inferior model to evaluate or select an unprecedentedly-powerful model. 

% and that neural models still strongly under-perform human evaluation \citep{evaluating-the-evaluation-2021}. 

%\textbf{Evaluating diversity, creativity, and novelty of LLMs.}
%
%With the increasing 
How language models differ from humans in terms of diversity, creativity, and novelty remains open due to the difficulty in evaluating semantic diversity at scale. \citet{raven-novelty-2023} study whether LLMs can generate novel outputs, where novelty is defined in terms of syntactic constructs such as parse trees and $n$-grams not present in the training corpus. \citet{rlhf-diversity-2023} study models from AlpacaFarm \citep{alpacafarm}, finding that RLHF tuned models are less diverse than SFT models according to lexical and neural metrics. \citet{vishakh-content-diversity-2023} find that when people use RLHF models to write essays, their essays contain less diverse content than a control group writing with a base LLM (their work measures semantic diversity by clustering key points in the text). \citet{young2024improving} propose a prompting strategy for increasing the structural diversity of poetry and programs. 
\citet{guo2024curious} perform a study on how recursively training on LLM generations reduces lexical and neural diversity of generations. 
%In contrast, we propose an open-ended task where we can automatically evaluate the semantic, lexical, and syntactic diversity.
% And most recently, it has recently been investigated using programs that LLMs like \textsc{GPT-4} substantially underperform humans in their definition of creativity \alex{todo: review more}.

% Finally, recent work has studied diversity of LLMs for code \citep{guo2024curious,young2024improving}; however, our focus is on using code to prove semantic diversity of LLMs more broadly. \alex{review these for myself}



==> latex/sections/controlling_coh.tex <==
\input{latex/tables/coh_only_meta}
\subsection{Diversity When Controlling For Coherence} 
\label{subsec:coherent_analysis}

Generally, avoiding writing well-formed programs (i.e., without syntax and runtime errors) provides a good starting point for improving semantic diversity. In \Cref{tab:model_comparisons}, we report results for the subset of generations without syntax or runtime errors. 

\textbf{Semantic diversity does not increase.} When restricting to coherent programs, we find that instruction-tuning, increasing model size, and using few-shot prompting does not increase the semantic diversity. These results suggest that higher proportions of well-formed programs drive increases in diversity found above. Significantly as well, \textit{we find no evidence} that instruction-tuning or larger models \textit{reduce} semantic diversity.

\textbf{Preference-tuning reduces diversity of form.}
%
We find that preference tuning reduces syntactic and lexical diversity, whereas syntactic and lexical diversity is somewhat greater in the SFT \codellama models.

==> latex/sections/on_diversity.tex <==
\section{On Diversity}

Talk about diversity here (maybe related?)

==> latex/tables/all_programs.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[!ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{l|l|c|cc|cc|cc|cc}
    \toprule
    & & & \multicolumn{2}{c|}{\textbf{Coh.}} & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Dist-N}} & \multicolumn{2}{c}{\textbf{CAST}} \\
    \cmidrule{4-11}
    \textbf{Comparison} & \textbf{Model} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
    \midrule
    \textsc{Base vs. Inst.} & \textsc{All Open} & 21 & \underline{0.001} & \underline{0.863} & \underline{0.002} & \underline{0.985} & \underline{<0.001} & \underline{-1.964} & \underline{<0.001} & \underline{-1.096} \\
    \textsc{Base vs. Inst.} & \textsc{CodeLlama} & 9 & \underline{0.039} & 0.579 & \underline{0.020} & 0.454 & 0.164 & -0.749 & 0.203 & -0.278 \\
    \textsc{Base vs. Inst.} & \textsc{Llama3 \& Llama3.1} & 12 & \underline{0.016} & \underline{1.049} & \underline{0.027} & \underline{1.387} & \underline{<0.001} & \underline{-3.987} & \underline{<0.001} & \underline{-1.932} \\
    \textsc{Base vs. Inst.} & \textsc{Llama3} & 6 & \underline{0.031} & \underline{1.979} & \underline{0.031} & \underline{2.154} & \underline{0.031} & \underline{-3.026} & \underline{0.031} & \underline{-1.834} \\
    \textsc{Base vs. Inst.} & \textsc{Llama3.1} & 6 & 0.563 & \underline{0.814} & 0.563 & \underline{0.822} & \underline{0.031} & \underline{-5.705} & \underline{0.031} & \underline{-1.962} \\
    \textsc{Base vs. Inst.} & \textsc{All Open (Best Coh.)} & 6 & \underline{0.028} & \underline{1.073} & \underline{0.028} & \underline{1.609} & \underline{0.028} & \underline{-1.862} & \underline{0.046} & \underline{-1.414} \\
    \textsc{Base vs. Inst.} & \textsc{All Open (Best Sem.)} & 6 & \underline{0.028} & \underline{1.130} & \underline{0.028} & \underline{1.652} & 0.075 & \underline{-1.467} & 0.116 & \underline{-0.811} \\
    \midrule
    \textsc{Small vs. Large} & \textsc{All Open} & 18 & 0.108 & 0.151 & \underline{0.001} & 0.515 & \underline{0.038} & 0.353 & 0.108 & 0.287 \\
    \textsc{Small vs. Large} & \textsc{Base} & 9 & 0.570 & 0.154 & 0.098 & 0.506 & 0.570 & 0.015 & 0.910 & 0.099 \\
    \textsc{Small vs. Large} & \textsc{Instruct} & 9 & 0.203 & 0.180 & \underline{0.012} & 0.688 & \underline{0.004} & \underline{0.817} & \underline{0.039} & 0.522 \\
    \textsc{Small vs. Large} & \textsc{Commercial} & 18 & 0.579 & 0.237 & 0.212 & 0.425 & 0.284 & -0.496 & 0.495 & -0.282 \\
    \midrule
    \textsc{ZS vs. FS} & \textsc{All} & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \underline{0.002} & -0.450 & \underline{<0.001} & \underline{-1.414} \\
    \textsc{ZS vs. FS} & \textsc{Base} & 7 & \underline{0.016} & \underline{2.575} & \underline{0.016} & \underline{7.020} & \underline{0.047} & -0.794 & \underline{0.016} & \underline{-6.751} \\
    \textsc{ZS vs. FS} & \textsc{Instruct} & 7 & 1.000 & 0.087 & 0.297 & -0.525 & 0.109 & -0.619 & \underline{0.047} & \underline{-0.998} \\
    \textsc{ZS vs. FS} & \textsc{Commercial} & 7 & 0.813 & 0.246 & 0.742 & -0.077 & 0.055 & -0.444 & \underline{0.008} & \underline{-1.201} \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Significance and Effect Size Tests for All Comparisons.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}. Metrics: Coherence (Coh.), Semantic Diversity (Sem.), Syntactic Diversity (Dist-N), Lexical Diversity (CAST). Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.8 (large effect size). p-values < 0.001 are reported as ``<0.001". Comparisons: Base vs. Instruct (Base vs. Inst.), Small vs. Large, Zero-Shot vs. Few-Shot (ZS vs. FS). \textsc{Best Coh.} and \textsc{Best Sem.} are paired comparisons when choosing the best Model $\times$ Prompt pair for the given}
    \label{tab:all_comparisons}
\end{table*}

==> latex/tables/coh_only_all_comparisons.tex <==
\begin{table*}[!ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{l|l|c|cc|cc|cc}
    \toprule
    & & & \multicolumn{2}{c|}{\textbf{Semantic Diversity}} & \multicolumn{2}{c|}{\textbf{Syntactic Diversity}} & \multicolumn{2}{c}{\textbf{Lexical Diversity}} \\
    \cmidrule{4-9}
    \textbf{Comparison} & \textbf{Model} & \textbf{Size} & \textbf{p} & \textbf{Cohen's d} & \textbf{p} & \textbf{Cohen's d} & \textbf{p} & \textbf{Cohen's d} \\
    \midrule
    \multirow{6}{*}{\textsc{Base vs. Instruct}} & All Open & 21 & 0.708 & -0.051 & \underline{0.083} & \underline{-0.527} & \underline{0.083} & \underline{-0.548} \\
    & CodeLLama & 9 & 0.570 & 0.040 & 0.426 & 0.474 & 0.570 & 0.386 \\
    & MetaLLama & 12 & 0.910 & -0.125 & \underline{0.001} & \underline{-1.886} & \underline{0.005} & \underline{-1.624} \\
    & MetaLLama3 & 6 & 0.688 & -0.268 & \underline{0.031} & \underline{-2.023} & \underline{0.063} & \underline{-2.143} \\
    & MetaLlama3.1 & 6 & 1.000 & -0.006 & \underline{0.063} & \underline{-1.606} & \underline{0.063} & \underline{-1.139} \\
    & All Open (Best Coh) & 6 & \underline{0.075} & 0.079 & \underline{0.046} & \underline{-1.566} & \underline{0.028} & \underline{-1.608} \\
    & All Open (Best Sem.) & 6 & 0.345 & 0.030 & 0.116 & \underline{-1.224} & \underline{0.028} & \underline{-1.276} \\
    \midrule
    \multirow{4}{*}{\textsc{Small vs. Large}} & All Open & 18 & 0.332 & 0.134 & \underline{0.039} & 0.462 & 0.098 & 0.420 \\
    & Base & 9 & 0.401 & 0.238 & 0.176 & 0.176 & 0.461 & 0.130 \\
    & Instruct & 9 & 0.734 & 0.013 & 0.098 & \underline{0.813} & 0.129 & \underline{0.733} \\
    & Commercial* & 18 & 0.890 & -0.109 & 0.454 & -0.470 & 0.330 & -0.381 \\
    \midrule
    \multirow{4}{*}{\textsc{ZS vs. FS}} & All & 21 & \underline{0.015} & \underline{-0.501} & 0.869 & 0.146 & 0.927 & 0.115 \\
    & Base & 7 & 0.688 & -0.308 & 0.156 & \underline{1.336} & 0.094 & \underline{1.353} \\
    & Instruct & 7 & 0.219 & \underline{-0.554} & 0.813 & -0.249 & 0.813 & -0.220 \\
    & Commercial & 7 & \underline{0.028} & \underline{-0.682} & 0.219 & \underline{-0.686} & 0.156 & \underline{-0.731} \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Significance and Effect Size Tests for Various Model Comparisons.} Results show p-values from Wilcoxon's Signed-Rank Test and Effect Size measured by Cohen's d. Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.5 (medium to large effect size). Comparisons include Base vs. Instruct models, Small vs. Large models, and Zero-Shot vs. Few-Shot (ZS vs. FS) approaches. *For Commercial models, cost-per-token is used as a proxy for model size.}
    \label{tab:model_comparisons}
\end{table*}

==> latex/tables/coh_only_meta.tex <==
\begin{table*}[!t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{l|l|c|cc|cc|cc}
    \toprule
    & & & \multicolumn{2}{c|}{\textbf{Semantic}} & \multicolumn{2}{c|}{\textbf{Syntactic}} & \multicolumn{2}{c}{\textbf{Lexical}} \\
    \cmidrule{4-9}
    \textbf{Comparison} & \textbf{Model} & \textbf{Size} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
    \midrule
    \multirow{7}{*}{\textsc{Base vs. Instruct}} & \textsc{All Open} & 21 & 0.708 & -0.051 & 0.083 & -0.527 & 0.083 & -0.548 \\
    & \textsc{All Open (Best Coh)} & 6 & 0.075 & 0.079 & \textbf{0.046} & \textbf{-1.566} & \textbf{0.028} & \textbf{-1.608} \\
    & \textsc{All Open (Best Sem.)} & 6 & 0.345 & 0.030 & 0.116 & \textbf{-1.224} & \textbf{0.028} & \textbf{-1.276} \\
    & \textsc{CodeLLama} (\textbf{SFT}) & 9 & 0.570 & 0.040 & 0.426 & 0.474 & 0.570 & 0.386 \\
    & \textsc{LLama3 \& Llama3.1} (\textbf{PT}) & 12 & 0.910 & -0.125 & \textbf{0.001} & \textbf{-1.886} & \textbf{0.005} & \textbf{-1.624} \\
    & \textsc{LLama3} (\textbf{PT}) & 6 & 0.688 & -0.268 & \textbf{0.031} & \textbf{-2.023} & 0.063 & \textbf{-2.143} \\
    & \textsc{Llama3.1} (\textbf{PT})& 6 & 1.000 & -0.006 & 0.063 & \textbf{-1.606} & 0.063 & \textbf{-1.139} \\
    \midrule
    \multirow{4}{*}{\textsc{Small vs. Large}} & \textsc{All Open} & 18 & 0.332 & 0.134 & \textbf{0.039} & 0.462 & 0.098 & 0.420 \\
    & \textsc{Base} & 9 & 0.401 & 0.238 & 0.176 & 0.176 & 0.461 & 0.130 \\
    & \textsc{Instruct} & 9 & 0.734 & 0.013 & 0.098 & \textbf{0.813} & 0.129 & 0.733 \\
    & \textsc{Commercial}* & 18 & 0.890 & -0.109 & 0.454 & -0.470 & 0.330 & -0.381 \\
    \midrule
    \multirow{4}{*}{\textsc{ZS vs. FS}} & \textsc{All} & 21 & \textbf{0.015} & -0.501 & 0.869 & 0.146 & 0.927 & 0.115 \\
    & \textsc{Base} & 7 & 0.688 & -0.308 & 0.156 & \textbf{1.336} & 0.094 & \textbf{1.353} \\
    & \textsc{Instruct} & 7 & 0.219 & -0.554 & 0.813 & -0.249 & 0.813 & -0.220 \\
    & \textsc{Commercial} & 7 & \textbf{0.028} & -0.682 & 0.219 & -0.686 & 0.156 & -0.731 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Restricting to Coherent Generations.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}.  Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). }
    \label{tab:model_comparisons}
\end{table*}


% \begin{table*}[!t]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{3.0pt}
%     \begin{tabular}{l|l|c|cc|cc|cc}
%     \toprule
%     & & & \multicolumn{2}{c|}{\textbf{Semantic}} & \multicolumn{2}{c|}{\textbf{Syntactic}} & \multicolumn{2}{c}{\textbf{Lexical}} \\
%     \cmidrule{4-9}
%     \textbf{Comparison} & \textbf{Model} & \textbf{Size} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     \multirow{7}{*}{\textsc{Base vs. Instruct}} & \textsc{All Open} & 21 & 0.708 & -0.051 & 0.083 & \textbf{-0.527} & 0.083 & \textbf{-0.548} \\
%     & \textsc{All Open (Best Coh)} & 6 & 0.075 & 0.079 & \textbf{0.046} & \textbf{-1.566} & \textbf{0.028} & \textbf{-1.608} \\
%     & \textsc{All Open (Best Sem.)} & 6 & 0.345 & 0.030 & 0.116 & \textbf{-1.224} & \textbf{0.028} & \textbf{-1.276} \\
%     & \textsc{CodeLLama} & 9 & 0.570 & 0.040 & 0.426 & 0.474 & 0.570 & 0.386 \\
%     & \textsc{LLama3 \& Llama3.1} & 12 & 0.910 & -0.125 & \textbf{0.001} & \textbf{-1.886} & \textbf{0.005} & \textbf{-1.624} \\
%     & \textsc{LLama3} & 6 & 0.688 & -0.268 & \textbf{0.031} & \textbf{-2.023} & 0.063 & \textbf{-2.143} \\
%     & \textsc{Llama3.1} & 6 & 1.000 & -0.006 & 0.063 & \textbf{-1.606} & 0.063 & \textbf{-1.139} \\
%     % & \textsc{All Open (Best Coh)} & 6 & 0.075 & 0.079 & \textbf{0.046} & \textbf{-1.566} & \textbf{0.028} & \textbf{-1.608} \\
%     % & \textsc{All Open (Best Sem.)} & 6 & 0.345 & 0.030 & 0.116 & \textbf{-1.224} & \textbf{0.028} & \textbf{-1.276} \\
%     \midrule
%     \multirow{4}{*}{\textsc{Small vs. Large}} & \textsc{All Open} & 18 & 0.332 & 0.134 & \textbf{0.039} & 0.462 & 0.098 & 0.420 \\
%     & \textsc{Base} & 9 & 0.401 & 0.238 & 0.176 & 0.176 & 0.461 & 0.130 \\
%     & \textsc{Instruct} & 9 & 0.734 & 0.013 & 0.098 & \textbf{0.813} & 0.129 & \textbf{0.733} \\
%     & \textsc{Commercial}* & 18 & 0.890 & -0.109 & 0.454 & -0.470 & 0.330 & -0.381 \\
%     \midrule
%     \multirow{4}{*}{\textsc{ZS vs. FS}} & \textsc{All} & 21 & \textbf{0.015} & \textbf{-0.501} & 0.869 & 0.146 & 0.927 & 0.115 \\
%     & \textsc{Base} & 7 & 0.688 & -0.308 & 0.156 & \textbf{1.336} & 0.094 & \textbf{1.353} \\
%     & \textsc{Instruct} & 7 & 0.219 & \textbf{-0.554} & 0.813 & -0.249 & 0.813 & -0.220 \\
%     & \textsc{Commercial} & 7 & \textbf{0.028} & \textbf{-0.682} & 0.219 & \textbf{-0.686} & 0.156 & \textbf{-0.731} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Significance and Effect Size Tests for the Subset of Coherent Generations.} Results show p-values from Wilcoxon's Signed-Rank Test \textbf{W (p)}, and Effect Size measured by Cohen's d: \textbf{ES (d)}. Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8. Comparisons include Base vs. Instruct models, Small vs. Large models, and Zero-Shot vs. Few-Shot (ZS vs. FS) approaches. *For Commercial models, cost-per-token is used as a proxy for model size.\alex{effect size >0.5 is bold instead of 0.8} \alex{columns are swapped it seems? previously lexical went first }}
%     \label{tab:model_comparisons}
% \end{table*}

% \begin{table*}[!t]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{3.0pt}
%     \begin{tabular}{l|l|c|cc|cc|cc}
%     \toprule
%     & & & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Syn.}} & \multicolumn{2}{c}{\textbf{Lex.}} \\
%     \cmidrule{4-9}
%     \textbf{Comparison} & \textbf{Model} & \textbf{Size} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     \multirow{7}{*}{\textsc{Base vs. Instruct}} & \textsc{All Open} & 21 & 0.708 & -0.051 & 0.083 & \underline{-0.527} & 0.083 & \underline{-0.548} \\
%     & \textsc{CodeLLama} & 9 & 0.570 & 0.040 & 0.426 & 0.474 & 0.570 & 0.386 \\
%     & \textsc{MetaLLama} & 12 & 0.910 & -0.125 & \underline{0.001} & \underline{-1.886} & \underline{0.005} & \underline{-1.624} \\
%     & \textsc{MetaLLama3} & 6 & 0.688 & -0.268 & \underline{0.031} & \underline{-2.023} & 0.063 & \underline{-2.143} \\
%     & \textsc{MetaLlama3.1} & 6 & 1.000 & -0.006 & 0.063 & \underline{-1.606} & 0.063 & \underline{-1.139} \\
%     & \textsc{All Open (Best Coh)} & 6 & 0.075 & 0.079 & \underline{0.046} & \underline{-1.566} & \underline{0.028} & \underline{-1.608} \\
%     & \textsc{All Open (Best Sem.)} & 6 & 0.345 & 0.030 & 0.116 & \underline{-1.224} & \underline{0.028} & \underline{-1.276} \\
%     \midrule
%     \multirow{4}{*}{\textsc{Small vs. Large}} & \textsc{All Open} & 18 & 0.332 & 0.134 & \underline{0.039} & 0.462 & 0.098 & 0.420 \\
%     & \textsc{Base} & 9 & 0.401 & 0.238 & 0.176 & 0.176 & 0.461 & 0.130 \\
%     & \textsc{Instruct} & 9 & 0.734 & 0.013 & 0.098 & \underline{0.813} & 0.129 & \underline{0.733} \\
%     & \textsc{Commercial}* & 18 & 0.890 & -0.109 & 0.454 & -0.470 & 0.330 & -0.381 \\
%     \midrule
%     \multirow{4}{*}{\textsc{ZS vs. FS}} & \textsc{All} & 21 & \underline{0.015} & \underline{-0.501} & 0.869 & 0.146 & 0.927 & 0.115 \\
%     & \textsc{Base} & 7 & 0.688 & -0.308 & 0.156 & \underline{1.336} & 0.094 & \underline{1.353} \\
%     & \textsc{Instruct} & 7 & 0.219 & \underline{-0.554} & 0.813 & -0.249 & 0.813 & -0.220 \\
%     & \textsc{Commercial} & 7 & \underline{0.028} & \underline{-0.682} & 0.219 & \underline{-0.686} & 0.156 & \underline{-0.731} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Significance and Effect Size Tests for the Subset of Coherent Generations.} Results show p-values from Wilcoxon's Signed-Rank Test \textbf{W (p)}, and Effect Size measured by Cohen's d: \textbf{ES (d)}. Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.5 (medium to large effect size). Comparisons include Base vs. Instruct models, Small vs. Large models, and Zero-Shot vs. Few-Shot (ZS vs. FS) approaches. *For Commercial models, cost-per-token is used as a proxy for model size.\alex{effect size >0.5 is underlined instead of 0.8}}
%     \label{tab:model_comparisons}
% \end{table*}

==> latex/tables/humaneval.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

% \begin{table*}[!h]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{2pt}
%     \arrayrulecolor{blue} % Set table borders to blue
%     \begin{tabularx}{\textwidth}{c|*{1}{Y}|*{1}{Y}}
%     \toprule

%        & \multicolumn{1}{c|}{\textbf{Base Model}} & \multicolumn{1}{c}{\textbf{Instruction-Tuned}} \\
%     \midrule
%     % \textbf{Model} & \textbf{Coh.} & \textbf{Sem.} & \textbf{Syn.} & \textbf{Lex.} & \textbf{ $\Delta$ Coh.} & \textbf{ $\Delta$ Sem.} & \textbf{ $\Delta$ Syn.} & \textbf{ $\Delta$ Lex.} \\
%     \toprule
%     \textsc{CodeLlama-7B}  & 33.5 & 34.8 \\
%     \textsc{CodeLlama-34B} & 48.8 & 41.5 \\
%     \textsc{CodeLlama-70B} & 53.0 & 67.8 \\
%     \midrule
%     \textsc{Meta-Llama-3-8B} & 37.2 & 60.4 \\
%     \textsc{Meta-Llama-3-70B} & 58.5 & 81.7 \\
%     \midrule
%     \textsc{Meta-Llama-3.1-8B} & - & 72.6 \\
%     \textsc{Meta-Llama-3.1-70B} & - & 80.5 \\
%     \bottomrule

%     \end{tabularx}
%     \caption{\reb{\label{tab:base_vs_instruct_humaneval} Pass@1 performance of all tested models on HumanEval benchmark (0-Shot).}}
% \end{table*}

\begin{table}[h]
  \center
   \setlength{\tabcolsep}{3pt}
   \arrayrulecolor{blue} % Set table borders to blue
  \begin{tabular}{lr|cc} 
  \toprule
  \textbf{Model} &\multicolumn{1}{c}{\textbf{Size}}& \multicolumn{2}{c}{Code Generation Benchmarks} \\  
  && \textbf{HumanEval} & \textbf{MBPP} \\ 
  \midrule
  \multirow{3}{*}{\codellama} 
  & 7B  & 33.5 & 41.4 \\
  &34B  & 48.8 & 55.0 \\
  &70B  & 53.0 & 62.4 \\
  \midrule
  \multirow{3}{*}{\codellamainst} 
  &7B  & 34.8 & 44.4 \\
  &34B  & 41.5 & 57.0 \\
  &70B  & 67.8 & 62.2 \\
  \midrule
  \multirow{3}{*}{\codellamapy} 
  &7B  & 38.4 & 47.6 \\
  &34B  & 53.7 & 56.2 \\
  &70B  & 57.3 & 65.6 \\
  \midrule
  \midrule
  \multirow{2}{*}{\llamathree}
  &8B  & 37.2 & - \\
  &70B  & 58.5 & - \\
  \midrule
  \multirow{2}{*}{\llamathreeone}
  &8B  & 8.5 & 47.6 \\
  &70B  & - & 66.2 \\
  \midrule
  % \multirow{1}{*}{Mistral}
  % &7B  & 30.5  & 47.5 \\
  % \multirow{1}{*}{Mixtral}
  % &8$\times$22B  & 45.1 & 71.2 \\
  % \cmidrule[1.3pt]{1-4} % Adjusted thicker line
  \multirow{2}{*}{\llamathreeinst} 
  &8B  & 60.4 & 70.6 \\
  &70B  & 81.7 & 82.5 \\
  \midrule
  \multirow{2}{*}{\llamathreeoneinst} 
  &8B  & 72.6 & 72.8 \\
  &70B  & 80.5 & 86.0 \\
  % \midrule
  % \multirow{1}{*}{Mistral-Instruct}
  % &7B  & 40.2 & 49.5 \\
  % \multirow{1}{*}{Mixtral-Instruct}
  % &8$\times$22B  & 75.6 & 78.6 \\
  \midrule
  \midrule
  \multirow{3}{*}{Qwen2.5-Coder} 
  & 7B  & 61.6 & 76.9 \\
  &14B  & 64.0 & 81.0 \\
  &32B  & 65.9 & 83.0 \\
  \midrule
  \multirow{3}{*}{Qwen2.5-Coder-Instruct} 
  &7B  & 88.4 & 83.5 \\
  &14B  & 89.6 & 86.2 \\
  &32B  & 92.7 & 90.2 \\
  \midrule
  \midrule
  \multirow{1}{*}{\texttt{code-davinci-002}}
  &  & 47.0 & 58.10 \\
  \multirow{1}{*}{\texttt{gpt-3.5-turbo-0125}}
  &  & 48.1 & - \\
  \multirow{1}{*}{\texttt{gpt-3.5-turbo-instruct}}
  &  & 68.0 & 82.0 \\
  \multirow{1}{*}{\texttt{gpt-4o-mini}}
  &  & 87.2 & - \\
  \cmidrule[1.3pt]{1-4} % Adjusted thicker line
  \multirow{1}{*}{Claude 3 Sonnet}
  &  & 73.0 & 79.4 \\
  \multirow{1}{*}{Claude 3 Haiku}
  &  & 75.9 & 80.4 \\
  \bottomrule
  \end{tabular}
  \caption{\reb{\textbf{Pass@1 scores on HumanEval and MBPP.} Results for the models as provided by~\cite{codellama-2023} (\codellama), \cite{llama3-2024} (\llamathree, \llamathreeone, Mistral, \texttt{gpt-3.5-turbo-instruct}), \cite{qwen} (Qwen2.5-Coder), \cite{zheng2023survey} (\texttt{code-davinci-002}), \cite{achiam2023gpt} (\texttt{gpt-3.5-turbo-0125}, \texttt{gpt-4o-mini}), and \cite{anthropic2024claude3} (Claude 3).}}
\label{tab:correctness}
\end{table}


==> latex/tables/meta_results.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[!ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l|c|c|cc|cc|cc|cc}
    \toprule
    & & & \multicolumn{2}{c|}{\textbf{Coh.}} & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Dist-N}} & \multicolumn{2}{c}{\textbf{CAST}} \\
    \cmidrule{4-11}
    \textbf{Comparison} & \textbf{Subset} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
    \midrule
    Base vs. Instruct, All Open & All & 21 & \underline{0.001} & \underline{0.863} & \underline{0.002} & \underline{0.985} & \underline{<0.001} & \underline{-1.964} & \underline{<0.001} & \underline{-1.096} \\
    Base vs. Instruct, ``Best Prompt" & All & 6 & \underline{0.028} & \underline{1.073} & \underline{0.028} & \underline{1.609} & \underline{0.028} & \underline{-1.862} & \underline{0.046} & \underline{-1.414} \\
    Small vs. Large, All Open & All & 18 & 0.108 & 0.151 & \underline{0.001} & 0.515 & \underline{0.038} & 0.353 & 0.108 & 0.287 \\
    Zero-Shot vs. Two-Shot, All Models & All & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \underline{0.002} & -0.450 & \underline{<0.001} & \underline{-1.414} \\
    \midrule
    Base vs. Instruct, All & Coh. & 21 & --- & --- & 0.708 & -0.051 & 0.083 & -0.527 & 0.083 & -0.548 \\
    Base vs. Instruct, ``Best Prompt" & Coh. & 6 & --- & --- & 0.075 & 0.079 & \underline{0.046} & \underline{-1.566} & \underline{0.028} & \underline{-1.608} \\
    Small vs. Large, All Open & Coh. & 18 & --- & --- & 0.332 & 0.134 & \underline{0.039} & 0.462 & 0.098 & 0.420 \\
    Zero-Shot vs. Two-Shot, All Models & Coh. & 21 & --- & --- & \underline{0.015} & -0.501 & 0.869 & 0.146 & 0.927 & 0.115 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Meta Results Comparing Metric Differences.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}. Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.8 (large effect size). p-values < 0.001 are reported as ``<0.001". ``All" subset includes all samples, while ``Coh." subset includes only coherent samples.}
    \label{tab:meta_results}
\end{table*}

% \begin{table*}[!ht]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l|c|cc|cc|cc|cc}
%     \toprule
%     & & \multicolumn{2}{c|}{\textbf{Coh.}} & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Dist-N}} & \multicolumn{2}{c}{\textbf{CAST}} \\
%     \cmidrule{3-10}
%     \textbf{Comparison} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     Base vs. Instruct, All Open & 21 & \underline{0.001} & \underline{0.863} & \underline{0.002} & \underline{0.985} & \underline{<0.001} & \underline{-1.964} & \underline{<0.001} & \underline{-1.096} \\
%     Base vs. Instruct, ``Best Prompt" & 6 & \underline{0.028} & \underline{1.073} & \underline{0.028} & \underline{1.609} & \underline{0.028} & \underline{-1.862} & \underline{0.046} & \underline{-1.414} \\
%     Small vs. Large, All Open & 18 & 0.108 & 0.151 & \underline{0.001} & 0.515 & \underline{0.038} & 0.353 & 0.108 & 0.287 \\
%     Zero-Shot vs. Two-Shot, All Models & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \underline{0.002} & -0.450 & \underline{<0.001} & \underline{-1.414} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Meta Results Comparing Metric Differences.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}. Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.8 (large effect size). p-values < 0.001 are reported as ``<0.001".}
%     \label{tab:meta_results}
% \end{table*}


% \begin{table*}[!htbp]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l|c|cc|cc|cc|cc}
%     \toprule
%     & & \multicolumn{2}{c|}{\textbf{Coh.}} & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Dist-N}} & \multicolumn{2}{c}{\textbf{CAST}} \\
%     \cmidrule{3-10}
%     \textbf{Comparison} & \textbf{Size} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     Base vs. Instruct (All open) & 21 & \underline{0.001} & \underline{\textbf{0.863}} & \underline{0.002} & \underline{\textbf{0.985}} & \underline{<0.001} & \underline{\textbf{-1.964}} & \underline{<0.001} & \underline{\textbf{-1.096}} \\
%     Base vs. Instruct (``Best Prompt") & 6 & \underline{0.028} & \underline{\textbf{1.073}} & \underline{0.028} & \underline{\textbf{1.609}} & \underline{0.028} & \underline{\textbf{-1.862}} & \underline{0.046} & \underline{\textbf{-1.414}} \\
%     Small vs. Large (All Open) & 18 & 0.108 & \textbf{0.151} & \underline{0.001} & \textbf{0.515} & \underline{0.038} & \textbf{0.353} & 0.108 & \textbf{0.287} \\
%     Default vs. Two Shot (All Models) & 21 & 0.055 & \textbf{0.055} & 1.000 & \textbf{0.017} & \underline{0.002} & \textbf{-0.450} & \underline{<0.001} & \underline{\textbf{-1.414}} \\
%     \bottomrule
%     \end{tabular}
%     \caption{Results from Wilcoxon's Signed-Rank Test p-values (\textbf{W (p)}) and Effect Size measured by Cohen's D (\textbf{ES (d)}). Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.8 (large effect size).}
%     \label{tab:comparison}
% \end{table*}

% \begin{table*}[!htbp]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l|c|cc|cc|cc|cc}
%     \toprule
%     & & \multicolumn{2}{c|}{\textbf{Coh.}} & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Dist-N}} & \multicolumn{2}{c}{\textbf{CAST}} \\
%     \cmidrule{3-10}
%     \textbf{Comparison} & \textbf{Size} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     Base vs. Instruct (All open) & 21 & \underline{0.001} & \underline{0.863} & \underline{0.002} & \underline{0.985} & \underline{0.000} & \underline{-1.964} & \underline{0.000} & \underline{-1.096} \\
%     % \midrule
%     Base vs. Instruct (``Best Prompt") & 6 & \underline{0.028} & \underline{1.073} & \underline{0.028} & \underline{1.609} & \underline{0.028} & \underline{-1.862} & \underline{0.046} & \underline{-1.414} \\
%     % \midrule
%     Small vs. Large (All Open) & 18 & 0.108 & 0.151 & \underline{0.001} & 0.515 & \underline{0.038} & 0.353 & 0.108 & 0.287 \\
%     % \midrule
%     Default vs. Two Shot (All Models) & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \underline{0.002} & -0.450 & \underline{0.000} & \underline{-1.414} \\
%     \bottomrule
%     \end{tabular}
%     \caption{Results from Wilcoxon's Signed-Rank Test p-values (\textbf{W (p)}) and Effect Size measured by Cohen's D (\textbf{ES (d)}). Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.8 (large effect size).}
%     \label{tab:comparison}
% \end{table*}



% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \begin{table*}[!htbp]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l|c|cc|cc|cc|cc}
%     \toprule
%     & & \multicolumn{2}{c|}{\textbf{Coherence}} & \multicolumn{2}{c|}{\textbf{Semantic Diversity}} & \multicolumn{2}{c|}{\textbf{Syntactic Diversity}} & \multicolumn{2}{c}{\textbf{Lexical Diversity}} \\
%     \cmidrule{3-10}
%     \textbf{Comparison} & \textbf{Size} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     Base vs. Instruct (All open) & 21 & \underline{0.001} & \underline{0.863} & \underline{0.002} & \underline{0.985} & \underline{0.000} & \underline{-1.964} & \underline{0.000} & \underline{-1.096} \\
%     \midrule
%     Base vs. Instruct (``Best Prompt") & 6 & \underline{0.028} & \underline{1.073} & \underline{0.028} & \underline{1.609} & \underline{0.028} & \underline{-1.862} & \underline{0.046} & \underline{-1.414} \\
%     \midrule
%     Small vs. Large (All Open) & 18 & 0.108 & 0.151 & \underline{0.001} & 0.515 & \underline{0.038} & 0.353 & 0.108 & 0.287 \\
%     \midrule
%     Default vs. Two Shot (All Models) & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \underline{0.002} & -0.450 & \underline{0.000} & \underline{-1.414} \\
%     \bottomrule
%     \end{tabular}
%     \caption{Results from Wilcoxon's Signed-Rank Test p-values (\textbf{W (p)}) and Effect Size measured a Cohen's D (\textbf{ ES (d)}). Underlined p-values are below 0.05, and underlined ES (d) values have an absolute value greater than 0.8.}
%     \label{tab:comparison}
% \end{table*}

==> latex/tables/models.tex <==
\begin{table}[t!]
  \center
   \setlength{\tabcolsep}{3pt}
  \begin{tabular}{lr|ccc|ccc} %ccr@{}}
  \toprule
  Model &\multicolumn{1}{c}{Size}& \multicolumn{3}{c}{HumanEval} & \multicolumn{3}{c}{MBPP} \\%& \multicolumn{2}{c}{APPS}\\  % 
  && pass@1 & pass@10 & pass@100 & pass@1 & pass@10 & pass@100 \\%& pass@10 & pass@100\\
  \midrule 
  code-cushman-001 &12B & $33.5$ & - & - & $45.9$ & - & -\\ 
  GPT-3.5 (ChatGPT) &-& $48.1$ & - & - & $52.2$ & - & - \\
  GPT-4 &-& $67.0$ & - & - & - & - & - \\
  PaLM &540B& $26.2$ & - & - & $36.8$ & - & -\\
  PaLM-Coder &540B& $35.9$ & - & $88.4$ & $47.0$ & - & - \\
  PaLM 2-S & - & $37.6$ & - & $88.4$ & $50.0$ & - & - \\ 
  StarCoder Base &15.5B & $30.4$ & - & - & $49.0$ & - & - \\
  StarCoder Python &15.5B & $33.6$ & - & - & $52.7$ & - & - \\
  StarCoder Prompted & 15.5B & $40.8$ & - & - & $49.5$ & - & - \\
  \midrule
  \multirow{ 4}{*}{\llamavtwo} 
  & 7B  & $12.2$  & $25.2$& $44.4$ & $20.8$ &$41.8$ & $65.5$\\
  &13B  & $20.1$  &$34.8$ & $61.2$ & $27.6$&$48.1$& $69.5$\\
  &34B  & $22.6$  &$47.0$ & $79.5$ & $33.8$&$56.9$& $77.6$\\
  &70B  &  $30.5$ &$59.4$ & $87.0$ &$45.4$ &$66.2$& $83.1$\\
  \midrule
  \multirow{ 4}{*}{\model} &7B  & $33.5$  & $59.6$& $85.9$ & $41.4$&$66.7$ & $82.5$\\
  &13B  & $36.0$  &$69.4$ & $89.8$ & $47.0$ &$71.7$& $87.1$\\
  &34B  & $48.8$  &$76.8$ & $93.0$& $55.0$&$76.2$& $86.6$\\
  & 70B & $53.0$ &$84.561$ &$96.241$ & $62.4$ &$81.061$ & $91.869$\\
  \midrule
  \multirow{ 4}{*}{\instmodel} &7B  &$34.756$  & $64.3$ & $88.1$ & $44.400$&$65.4$&  $76.8$\\
  &13B  & $42.683$ & $71.6$ & $91.6$ & $49.400$ &$71.2$&  $84.1$\\
  &34B  &  $41.5$& $77.2$ & $93.5$ & $57.0$ &$74.6$& $85.4$\\
  & 70B & $67.8$ & $90.3$& $97.257$& $62.2$ & $79.6$& $89.208$\\
  %\multirow{ 2}{*}{
  \textsc{Unnatural} \model
  %}
  &34B & $62.19512195121951$ & $85.17042359520399$& $95.43887547089229$&$61.2$&$76.5886525678425$&$86.6854745042413$\\
  \midrule
  % Base, Language specialized \\
  \multirow{ 4}{*}{\pymodel}& 7B  & $38.4$  &$70.3$ & $90.6$& $47.6$&$70.3$&$84.8$\\
  &13B  & $43.3$  &$77.4$ & $94.1$& $49.0$&$74.0$&$87.6$\\
  &34B  & $53.7$  & $82.8$& $94.7$& $56.2$&$76.4$&$88.2$\\
  & 70B & $57.3$ & $89.340$& $98.420$ & $65.6$ & $81.523$& $91.900$ \\
  \bottomrule
  \end{tabular}
  \caption{}
\end{table}

==> latex/tables/post_training.tex <==
\begin{table*}[!t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|c|cc|cc|cc|cc|cc}
    \toprule
    & & \multicolumn{2}{c|}{\textbf{Validity}} & \multicolumn{2}{c|}{\textbf{Semantic}} & \multicolumn{2}{c|}{\textbf{Syntactic}} & \multicolumn{2}{c|}{\textbf{Lexical}} & \multicolumn{2}{c}{\textbf{Neural}} \\
    \cmidrule{3-12}
    \textbf{Comparison} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
    \midrule
    \textsc{Base vs. Inst (All)} & 42 & \textbf{<0.001} & \textbf{1.33} & \textbf{<0.001} & \textbf{1.34} & \textbf{<0.001} & \textbf{-1.10} & \textbf{0.028} & -0.47 & \textbf{<0.001} & \textbf{-1.53} \\
    \textsc{Base vs. Inst-SFT} & 12 & \textbf{<0.001} & \textbf{1.37} & \textbf{<0.001} & \textbf{1.36} & 0.266 & -0.34 & 0.339 & 0.21 & 0.339 & -0.42 \\
    \textsc{Base vs. Inst-DPO} & 18 & \textbf{0.006} & \textbf{1.11} & \textbf{0.005} & \textbf{1.10} & \textbf{0.014} & -0.84 & \textbf{<0.001} & \textbf{-1.68} & \textbf{<0.001} & \textbf{-2.37} \\
    \textsc{Base vs. Inst-RL} & 15 & \textbf{<0.001} & \textbf{1.67} & \textbf{<0.001} & \textbf{1.54} & \textbf{0.012} & \textbf{-1.20} & \textbf{0.035} & -0.66 & \textbf{<0.001} & \textbf{-2.12} \\
    \textsc{Base vs. Inst-Pref} & 33 & \textbf{<0.001} & \textbf{1.34} & \textbf{<0.001} & \textbf{1.29} & \textbf{<0.001} & \textbf{-1.45} & \textbf{0.001} & -0.77 & \textbf{<0.001} & \textbf{-2.29} \\
    \midrule
    \textsc{SFT vs. DPO} & 12 & 0.151 & 0.51 & 0.266 & 0.39 & \textbf{<0.001} & \textbf{-0.90} & \textbf{0.003} & \textbf{-0.63} & \textbf{<0.001} & \textbf{-1.52} \\
    \textsc{SFT vs. RL} & 9 & \textbf{0.004} & \textbf{3.19} & \textbf{0.004} & \textbf{2.49} & \textbf{0.004} & \textbf{-2.43} & \textbf{0.004} & \textbf{-1.20} & \textbf{0.004} & \textbf{-2.29} \\
    \textsc{SFT vs. Pref} & 21 & \textbf{<0.001} & \textbf{0.97} & \textbf{0.002} & 0.77 & \textbf{<0.001} & \textbf{-1.30} & \textbf{<0.001} & \textbf{-0.83} & \textbf{<0.001} & \textbf{-1.86} \\
    \textsc{DPO vs. RL} & 9 & 1.0 & 0.10 & 0.301 & -0.14 & \textbf{0.039} & -0.60 & \textbf{0.004} & \textbf{-0.78} & 1.0 & -0.01 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Model Comparison Results.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}. Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). For effect sizes, negative values indicate the second model type in the comparison has lower values, while positive values indicate the second model type has higher values. "Inst" = Instruction-tuned, "Pref" combines RL and DPO models.}
    \label{tab:post_training}
\end{table*}

==> latex/tables/sm_v_lg.tex <==
% \begin{table*}[!ht]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{l|c|cc|cc|cc|cc|cc}
%     \toprule
%     & & \multicolumn{2}{c|}{\textbf{Validity}} & \multicolumn{2}{c|}{\textbf{Semantic}} & \multicolumn{2}{c|}{\textbf{Lexical}} & \multicolumn{2}{c|}{\textbf{Syntactic}} & \multicolumn{2}{c}{\textbf{Neural}} \\
%     \cmidrule{3-12}
%     \textbf{Comparison} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     \textsc{Sm. vs. Lg.} & 27 & \textbf{0.030} & 0.20 & \textbf{0.017} & 0.26 & 0.485 & 0.09 & 0.170 & 0.15 & 0.269 & 0.12 \\
%     \textsc{Sm. vs. Lg. Base} & 6 & 0.063 & 0.57 & 0.063 & 0.56 & 0.063 & 0.69 & 0.063 & 0.74 & \textbf{0.031} & \textbf{0.80} \\
%     \textsc{Sm. vs. Lg. Inst} & 21 & 0.111 & 0.20 & 0.070 & 0.27 & 0.539 & -0.11 & 0.683 & 0.06 & 0.759 & -0.05 \\
%     \textsc{Sm. vs. Lg. Pref} & 15 & 0.330 & 0.13 & 0.277 & 0.20 & 0.330 & -0.19 & 0.454 & 0.10 & 0.389 & 0.14 \\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Model Size Comparison Results.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with sample size \textbf{N}. Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). Positive effect sizes indicate higher values for small models, negative for large models. "Inst" = Instruction-tuned, "Pref" = Preference-optimized models.}
%     \label{tab:sm_v_lg}
% \end{table*}

\begin{table*}[!ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|c|cc|cc|cc|cc|cc}
    \toprule
    & & \multicolumn{2}{c|}{\textbf{Validity}} & \multicolumn{2}{c|}{\textbf{Semantic}} & \multicolumn{2}{c|}{\textbf{Syntactic}} & \multicolumn{2}{c|}{\textbf{Lexical}} & \multicolumn{2}{c}{\textbf{Neural}} \\
    \cmidrule{3-12}
    \textbf{Comparison} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
    \midrule
    \textsc{Sm. vs. Lg.} & 27 & \textbf{0.030} & 0.20 & \textbf{0.017} & 0.26 & 0.170 & 0.15 & 0.485 & 0.09 & 0.269 & 0.12 \\
    \textsc{Sm. vs. Lg. Base} & 6 & 0.063 & 0.57 & 0.063 & 0.56 & 0.063 & 0.74 & 0.063 & 0.69 & \textbf{0.031} & \textbf{0.80} \\
    \textsc{Sm. vs. Lg. Inst} & 21 & 0.111 & 0.20 & 0.070 & 0.27 & 0.683 & 0.06 & 0.539 & -0.11 & 0.759 & -0.05 \\
    \textsc{Sm. vs. Lg. Pref} & 15 & 0.330 & 0.13 & 0.277 & 0.20 & 0.454 & 0.10 & 0.330 & -0.19 & 0.389 & 0.14 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Model Size Comparison Results.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with sample size \textbf{N}. Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). Positive effect sizes indicate higher values for small models, negative for large models. "Inst" = Instruction-tuned, "Pref" = Preference-optimized models.}
    \label{tab:sm_v_lg}
\end{table*}

==> latex/tables/sm_v_lg_and_fs_all.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table*}[!ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{l|l|c|cc|cc|cc|cc}
    \toprule
    & & & \multicolumn{2}{c|}{\textbf{Coherence}} & \multicolumn{2}{c|}{\textbf{Semantic}} & \multicolumn{2}{c|}{\textbf{Syntactic}} & \multicolumn{2}{c}{\textbf{Lexical}} \\
    \cmidrule{4-11}
    \textbf{Comparison} & \textbf{Model} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
    \midrule
    \multirow{4}{*}{\textsc{Small vs. Large}} & \textsc{All Open} & 18 & 0.108 & 0.151 & \textbf{0.001} & 0.515 & \textbf{0.038} & 0.353 & 0.108 & 0.287 \\
    & \textsc{Base} & 9 & 0.570 & 0.154 & 0.098 & 0.506 & 0.570 & 0.015 & 0.910 & 0.099 \\
    & \textsc{Instruct} & 9 & 0.203 & 0.180 & \textbf{0.012} & 0.688 & \textbf{0.004} & \textbf{0.817} & \textbf{0.039} & 0.522 \\
    & \textsc{Commercial} & 18 & 0.579 & 0.237 & 0.212 & 0.425 & 0.284 & -0.496 & 0.495 & -0.282 \\
    \midrule
    \multirow{4}{*}{\textsc{ZS vs. FS}} & \textsc{All} & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \textbf{0.002} & -0.450 & \textbf{<0.001} & \textbf{-1.414} \\
    & \textsc{Base} & 7 & \textbf{0.016} & \textbf{2.575} & \textbf{0.016} & \textbf{7.020} & \textbf{0.047} & -0.794 & \textbf{0.016} & \textbf{-6.751} \\
    & \textsc{Instruct} & 7 & 1.000 & 0.087 & 0.297 & -0.525 & 0.109 & -0.619 & \textbf{0.047} & \textbf{-0.998} \\
    & \textsc{Commercial} & 7 & 0.813 & 0.246 & 0.742 & -0.077 & 0.055 & -0.444 & \textbf{0.008} & \textbf{-1.201} \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Model Size and Zero- vs. Few-Shot Comparisons.} Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}.  Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). For Commercial models, because model size is unknown, we use cost-per-token as a proxy and match models within the same family to the best of our ability. }
    % Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}. Metrics: Coherence (Coh.), Semantic Diversity (Sem.), Syntactic Diversity (Dist-N), Lexical Diversity (CAST). Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). p-values < 0.001 are reported as ``<0.001". 
    \label{tab:size_and_shot_comparisons}
\end{table*}


% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \begin{table*}[!ht]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{l|l|c|cc|cc|cc|cc}
%     \toprule
%     & & & \multicolumn{2}{c|}{\textbf{Coh.}} & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Lex.}} & \multicolumn{2}{c}{\textbf{Syn.}} \\
%     \cmidrule{4-11}
%     \textbf{Comparison} & \textbf{Model} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     \textsc{Small vs. Large} & \textsc{All Open} & 18 & 0.108 & 0.151 & \textbf{0.001} & 0.515 & \textbf{0.038} & 0.353 & 0.108 & 0.287 \\
%     \textsc{Small vs. Large} & \textsc{Base} & 9 & 0.570 & 0.154 & 0.098 & 0.506 & 0.570 & 0.015 & 0.910 & 0.099 \\
%     \textsc{Small vs. Large} & \textsc{Instruct} & 9 & 0.203 & 0.180 & \textbf{0.012} & 0.688 & \textbf{0.004} & \textbf{0.817} & \textbf{0.039} & 0.522 \\
%     \textsc{Budget vs. Cost}* & \textsc{Commercial}* & 18 & 0.579 & 0.237 & 0.212 & 0.425 & 0.284 & -0.496 & 0.495 & -0.282 \\
%     \midrule
%     \textsc{ZS vs. FS} & \textsc{All} & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \textbf{0.002} & -0.450 & \textbf{<0.001} & \textbf{-1.414} \\
%     \textsc{ZS vs. FS} & \textsc{Base} & 7 & \textbf{0.016} & \textbf{2.575} & \textbf{0.016} & \textbf{7.020} & \textbf{0.047} & -0.794 & \textbf{0.016} & \textbf{-6.751} \\
%     \textsc{ZS vs. FS} & \textsc{Instruct} & 7 & 1.000 & 0.087 & 0.297 & -0.525 & 0.109 & -0.619 & \textbf{0.047} & \textbf{-0.998} \\
%     \textsc{ZS vs. FS} & \textsc{Commercial} & 7 & 0.813 & 0.246 & 0.742 & -0.077 & 0.055 & -0.444 & \textbf{0.008} & \textbf{-1.201} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Significance and Effect Size Tests for Model Size and Shot Comparisons.} Comparisons: Small vs. Large (model size), Zero-Shot vs. Few-Shot (ZS vs. FS). *For Commercial models, because model size information is not transparent, we use the cost-per-token as a proxy for model size and attempt to match models within the same family to the best of our abilities. Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). }
%     % Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}. Metrics: Coherence (Coh.), Semantic Diversity (Sem.), Syntactic Diversity (Dist-N), Lexical Diversity (CAST). Bold p-values are below 0.05, and bold d-values have an absolute value greater than 0.8 (large effect size). p-values < 0.001 are reported as ``<0.001". 
%     \label{tab:size_and_shot_comparisons}
% \end{table*}

% \newcolumntype{Y}{>{\centering\arraybackslash}X}

% \begin{table*}[!ht]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{tabular}{l|l|c|cc|cc|cc|cc}
%     \toprule
%     & & & \multicolumn{2}{c|}{\textbf{Coh.}} & \multicolumn{2}{c|}{\textbf{Sem.}} & \multicolumn{2}{c|}{\textbf{Lex.}} & \multicolumn{2}{c}{\textbf{Syn.}} \\
%     \cmidrule{4-11}
%     \textbf{Comparison} & \textbf{Model} & \textbf{N} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} & \textbf{W (p)} & \textbf{ES (d)} \\
%     \midrule
%     \textsc{Small vs. Large} & \textsc{All Open} & 18 & 0.108 & 0.151 & \underline{0.001} & 0.515 & \underline{0.038} & 0.353 & 0.108 & 0.287 \\
%     \textsc{Small vs. Large} & \textsc{Base} & 9 & 0.570 & 0.154 & 0.098 & 0.506 & 0.570 & 0.015 & 0.910 & 0.099 \\
%     \textsc{Small vs. Large} & \textsc{Instruct} & 9 & 0.203 & 0.180 & \underline{0.012} & 0.688 & \underline{0.004} & \underline{0.817} & \underline{0.039} & 0.522 \\
%     \textsc{Budget vs. Cost}* & \textsc{Commercial}* & 18 & 0.579 & 0.237 & 0.212 & 0.425 & 0.284 & -0.496 & 0.495 & -0.282 \\
%     \midrule
%     \textsc{ZS vs. FS} & \textsc{All} & 21 & 0.055 & 0.055 & 1.000 & 0.017 & \underline{0.002} & -0.450 & \underline{<0.001} & \underline{-1.414} \\
%     \textsc{ZS vs. FS} & \textsc{Base} & 7 & \underline{0.016} & \underline{2.575} & \underline{0.016} & \underline{7.020} & \underline{0.047} & -0.794 & \underline{0.016} & \underline{-6.751} \\
%     \textsc{ZS vs. FS} & \textsc{Instruct} & 7 & 1.000 & 0.087 & 0.297 & -0.525 & 0.109 & -0.619 & \underline{0.047} & \underline{-0.998} \\
%     \textsc{ZS vs. FS} & \textsc{Commercial} & 7 & 0.813 & 0.246 & 0.742 & -0.077 & 0.055 & -0.444 & \underline{0.008} & \underline{-1.201} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Significance and Effect Size Tests for Model Size and Shot Comparisons.} Comparisons: Small vs. Large (model size), Zero-Shot vs. Few-Shot (ZS vs. FS). *For Commercial models, because model size information is not transparent, we use the cost-per-token as a proxy for model size and attempt to match models within the same family to the best of our abilities.}
%     % Results from Wilcoxon's Signed-Rank Test p-values: \textbf{W (p)}, and Effect Size measured by Cohen's D: \textbf{ES (d)} with paired sample size as \textbf{N}. Metrics: Coherence (Coh.), Semantic Diversity (Sem.), Syntactic Diversity (Dist-N), Lexical Diversity (CAST). Underlined p-values are below 0.05, and underlined d-values have an absolute value greater than 0.8 (large effect size). p-values < 0.001 are reported as ``<0.001". 
%     \label{tab:size_and_shot_comparisons}
% \end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

